The HiggsTools Handbook: Concepts and observables for deciphering the Nature of the Higgs Sector

This Report summarizes some of the activities of the HiggsTools Initial Training Network working group in the period 2015-2017. The main goal of this working group was to produce a document discussing various aspects of state-of-the-art Higgs physics at the Large Hadron Collider (LHC) in a pedagogic manner. The first part of the Report is devoted to a description of phenomenological searches for New Physics at the LHC. As the experimental measurements become more and more precise, there is a pressing need for a consistent framework in which deviations from the SM predictions can be computed precisely. We critically review the use of the \k{appa}-framework, fiducial and simplified template cross sections, effective field theories, pseudo-observables and phenomenological Lagrangians. In the second part of the Report, we propose $\varphi_{\eta}^*$ as a new and complementary observable for studying Higgs boson production at large transverse momentum in the case where the Higgs boson decays to two photons. We make a detailed study of the phenomenology of the $\varphi_{\eta}^*$ variable, contrasting the behaviour with the Higgs transverse momentum distribution using a variety of theoretical tools including event generators and fixed order perturbative computations.

==> intro_files/Introduction.tex <==
\section{Introduction}


The early discovery is certainly based on two pillars: experimental
analysis improvements and theory accuracy improvements.

The LHC data are consistent with the SM predictions for all the
parameterisations considered. Therefore, after the LHC Run 1, the SM of
particle physics has been completed, raising its status to that of a full
theory. However, despite its successes, this standard theory
has shortcomings vis-\`a-vis cosmological observations. At the same time,
there is presently a lack of direct evidence for new physics phenomena at
the accelerator energy frontier.
No matter what the LHC will uncover in the future, understanding the Higgs
boson properties is a pillar of the present paradigm. Direct searches,
thus possibly new physics, and precision measurements will have to be
consistent with each other. The need for a consistent theoretical
framework in which deviations from the SM predictions can be calculated is
necessary. Such a framework should be applicable to comprehensively
describe measurements in all sectors of particle physics, not only LHC
Higgs measurements but also electroweak precision data, etc. By
simultaneously describing all existing measurements, this framework then
becomes an intermediate step toward the next SM, hopefully revealing the
underlying symmetries.


==> phistar/BSM.tex <==
\section{Beyond the Standard Model}

The Standard Model has been extremely compatible with almost all the measurements made in particle physics experiments over the last few decades with no convincing hints of additional physics. However, despite its success so far, the Standard Model suffers theoretical shortcomings and also falls short of explaining several observations. This suggests that it cannot be the complete theory of nature, but rather serves as an effective theory of the energy limits we currently probe. One of the theoretical shortcomings of the SM is the unstable Higgs mass, which requires large cancellations between its bare mass and the quantum corrections from the particles that couple to it. New physics models that address this shortcoming predict new particles whose contributions to the loops can soften the unnatural fine tuning. These new particles are typically heavy resonances that couple strongly to the Higgs and can either be scalars, like in the case of supersymmetric models, or fermionic top parters, predicted by many composite Higgs models.

\input{BSMintro.tex} 

\subsection{Numerical Results}
\input{numerics.tex}


==> phistar/Taus.tex <==
\section{Taus}
\label{sec:taus}
%\textbf{Content}:\\
%Define what photons mean to an experimentalist. How do we see them, what properties do we measure, challenges/difficulties, advantages etc etc.\\
%Define how $\tau$ decays. How is it identified, which parts of detector are used, what is the biggest problem, what is the energy, angular resolution, what tools do the experimentalists use, discrimination power etc. \\
%MB and JC study whether the $\phi^*$ observable is relevant for $H \rightarrow \tau \tau$ analysis. They study the case when both the $\tau$s decay into electrons. Finally, a comparison of $\phi^*$ behaviour for  $H \rightarrow \tau \tau$ (GGF, VBF) and backgrounds ($Z \rightarrow \tau \tau$, W+Jet, top).
%Tools: A common subsection on tools used for these analyses. \\ 
%\\
%YB carries out a similar analysis for $\gamma \gamma$.\\
%\textbf{Tasks}:\\
%Gathering relevant literature and presenting it in a pedagogical manner. If a first year PhD student in experimental HEP reads this section, does s/he get a feel for what s/he will have to do to get started? Also contains plots and calculations by TM and MB\\
%\textbf{Authors}:\\TM, MB, YH?\\
%\textbf{Timeline}:\\December\\


\subsection{Tau leptons in a detector} \label{sec_taudet}

Tau leptons have a very short life time and, as a consequence, are not directly visible in a detector. Only the stable decay products are measured, and the presence of tau leptons then needs to be deduced from them. In the case of leptonic decays, electrons or muons are recorded (with transverse missing energy) and are directly identified as tau leptons in the analysis. On the other hand, hadronically decaying tau leptons require a specific treatment with reconstruction and subsequent identification \cite{ATLAS-CONF-2017-029}.

\subsection{$\phistar$ in the context of H$\rightarrow\tau\tau$ decays}

The $\phistar$ variable has initially been introduced to test QCD predictions in the context of Z/$\gamma^{*}\rightarrow e^{+}e^{-}$ and Z/$\gamma^{*}\rightarrow \mu^{+}\mu^{-}$ processes. It indeed enables to reduce experimental resolution compared to other dileptonic variables such as p$_{T}^{ll}$, the transverse momentum of the two leptons in the final state.\\
The aim of the section is to study and evaluate the impact of $\phistar$ in the case of H$\rightarrow\tau\tau$ decays. After having introduced the experimental context of this study, we will determine the experimental resolution of $\phistar$ for such a process, before eventually studying the potential discrimination power of this variable in the context of the search for SM H$\rightarrow\tau\tau$.

\subsubsection{Experimental context}

For the following studies, we used simulated data generated in the context of the ATLAS detector at LHC, for a center of mass energy of 13 TeV. The samples used were generated using two different Monte Carlo generators:
\begin{itemize}
\item PowHeg \cite{Frixione:2007vw}, for H$\rightarrow\tau\tau$ and top backgrounds (see section \ref{sec_discri}). Separate MC samples were generated for the main two Higgs boson production modes, ggF and VBF (VH and ttH are not considered in the following). This generator is interfaced with Pythia8 \cite{Sjostrand:2006za}: PowHeg deals with the hard scattering while Phythia8 performs the parton shower. The CT10\_AZNLOCTEQ6L1 \cite{Lai:2010vv} was used as PDF for H$\rightarrow\tau\tau$.
\item Sherpa 2.2.1 \cite{Gleisberg:2008ta}, for Z+jets backgrounds, with NNPDF30NNLO PDF tune. The Z+jets electroweak production is simulated separately using Sherpa 2.1.
\end{itemize}

A full simulation of the ATLAS detector by GEANT4 \cite{Agostinelli2003250} is applied to the samples produced with both generators.\\
\\
Tau leptons can decay either leptonically or hadronically, allowing three possible final states for the H$\rightarrow\tau\tau$ process: dileptonic, semi-leptonic and fully hadronic. The choice was made to perform our studies in the dileptonic final state, using both decays into electrons and muons. We therefore used reduced MC samples, on which a loose selection was applied in order to suppress events with non-dileptonic final state, while remaining inclusive enough to keep all the events we might be interested in.\\
These samples were then treated to match the experimental conditions of data recorded by the ATLAS detector during the early run 2 of LHC (2015 and 2016):
\begin{itemize}
\item The MC samples contain events generated for a whole range of number of pile-up events. Scale factors are then applied to each simulated event in order to match the actual pile-up distribution in data.
\item The simulation is not perfect, and does not reproduce exactly actual data. A whole set of scale factors are then determined in order to correct the simulated events, especially related to the reconstruction and identification of particles for hadronically decaying tau leptons). In this particular case of H$\rightarrow\tau_{lep}\tau_{lep}$, this scale factors are mainly related to leptons (electrons and muons) and jets.
\item The decision to keep a recorded event and to analyse it is taken by triggers, which are activated by the presence of the desired particle(s) with chosen kinematic conditions. In our case, lepton triggers for electrons and muons are used. These triggers are also applied to simulated events, and corresponding scale factors have to be applied in order to correct the difference of behaviour between actual and simulated data. 
\end{itemize}

\subsubsection{$\phi^{*}$ experimental resolution}

The paper \cite{Banfi:2010cf} compares, for Z/$\gamma^{*}\rightarrow e^{+}e^{-}$ and Z/$\gamma^{*}\rightarrow \mu^{+}\mu^{-}$, the experimental resolution of $\phi^{*}$ with some other dileptonic variables, in the context of the CDF and D0 detectors at Tevatron. We want here to reproduce some of these studies in the case of H$\rightarrow\tau_{lep}\tau_{lep}$ at ATLAS.\\

%\paragraph*{\textbf{$\mathbf{\phi^{*}}$ definition}}

%This variable is defined as:
%\begin{equation}
%\phi^{*} = tan(\phi_{acop})\times sin(\theta^{*})
%\end{equation}

%$\phi_{acop}$ depends only on the azimuthal angle between the two leptons, which is a common coordinate in ATLAS and is therefore directly available. $\theta^{*}$ has however to be defined. In hadron colliders analyses, it is commonly evaluated in the Collins Soper frame \cite{PhysRevD.16.2219}:
%\begin{equation}
%cos(\theta^{*}_{CS}) = \frac{sinh(\eta^{\ell-}-\eta^{\ell+})}{\sqrt{1+p_{T}^{\ell\ell}/m_{\ell\ell}}}\times\frac{2p_{T}^{\ell_{1}}p_{T}^{\ell_{2}}}{m_{\ell\ell}^{2}}
%\end{equation}
%with $m_{\ell\ell}$ the invariant mass of the two leptons, and $p_{T}^{\ell\ell}$ the vector sum of the two leptons.\\
%This definition however depends on transverse momenta measurement, which might impact negatively the resolution. Indeed angular directions are measured with a better resolution than momenta or energies. Following this statement, a new definition of $\theta^{*}$ was proposed, depending only on tracks directions:
%\begin{equation}
%cos(\theta^{*}_{\eta}) = tanh(\frac{\eta^{l-}-\eta^{l+}}{2})
%\end{equation}

%As a consequence to these two alternative definitions of $\theta^{*}$, we consider in the following the corresponding two definitions of $\phi^{*}$:
%\begin{equation}
%\phi^{*}_{\eta} = tan(\phi_{acop})\times sin(\theta^{*}_{CS})
%\end{equation}

%\begin{equation} \label{eq_phistar}
%\phi^{*}_{\eta} = tan(\phi_{acop})\times sin(\theta^{*}_{\eta})
%\end{equation}

%\paragraph*{\textbf{Experimental resolution}}

The experimental resolution is computed as the differences between a given variable at the reconstructed level and the same variable at the truth level. The detector effects are not taken into account at truth level and the exact properties of each particle in the process considered are therefore available.\\
In our case, we use both at reconstructed and truth level the electrons and muons coming from the tau leptons decays. All the other variables are derived from the basic properties of these particles, such as the dileptonic invariant mass and momentum.\\
The neutrinos from the tau leptons are therefore not taken into account here. At truth level the true tau leptons before decay are available, but comparing them with the reconstructed leptons would be unfair, since that would be adding a second effect on top of the experimental resolution.
% The studied tau leptons being boosted, one can argue that the neutrinos are produced in a direction close to the visible part of the decay, thus limiting the discrepancy between the directions of the mother tau and the daughter lepton. We would therefore expect $\theta^{*}_{\eta}$ to give a better resolution than $\theta^{*}_{CS}$ which should suffer from the missing neutrino momentum at reconstructed level.\\
%As a first step, we want to compare the resolutions of the two alternative $\theta^{*}$. The corresponding resolution distributions are given in Figure \ref{resol_thetastar}.\\

%\begin{figure}[h]
%    \centering
%    \begin{subfigure}[b]{0.49\textwidth}
%        \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_ggf_CutTrigger_CosThetaStar_resolution.eps}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.49\textwidth}
%        \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_ggf_CutTrigger_CosThetaStarCS_resolution.eps}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.49\textwidth}
%        \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_vbf_CutTrigger_CosThetaStar_resolution.eps}
%    \end{subfigure}
%    \begin{subfigure}[b]{0.49\textwidth}
%        \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_vbf_CutTrigger_CosThetaStarCS_resolution.eps}
%    \end{subfigure}
%   \caption{Experimental resolution of cos($\theta^{*}_{\eta}$) and cos($\theta^{*}_{CS}$), for ggF (top) and VBF (bottom) production modes. The distributions are normalised to 1.}
%    \label{resol_thetastar}
%\end{figure}

%It shows that cos($\theta^{*}_{\eta}$) provides a better resolution than cos($\theta^{*}_{CS}$), the distribution being much more peaked around zero. This observation is true for both the VBF and ggF Higgs boson production modes.\\
%These two $\theta^{*}_{\eta}$ result into two alternative definitions of $\phi^{*}$, whose resolution can also be compared. The corresponding distribution are given in Figure \ref{resol_phistar}. The better resolution of cos($\theta^{*}_{\eta}$) propagates to $\phi^{*}_{\eta}$, which is as a consequence better than $\phi^{*}_{CS}$. The two distribution are however much closer than those for cos($\theta^{*}$).\\
%From these checks, we can conclude that $\phi^{*}_{\eta}$ should be the privileged definition to be compared with with other dileptonic variable resolutions. We nonetheless keep $\phi^{*}_{CS}$ in the next studies for completeness.\\

$\phi^{*}_{\eta}$ depends only on tracks directions measurement, which are measured with high precision, especially compared to energies and momenta measurements.
On Figure \ref{phistar} are shown the $\phi^{*}_{\eta}$ distributions at reconstructed and truth level. The distributions are very close one to another, confirming that the effects of leptons' tracks measurement are quite small. We can then quantify this by computing $\phi^{*}_{\eta}$'s resolution. The distribution of the resolution is shown in Figure \ref{resol_phistar}.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_ggfphistar.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_vbfphistar.eps}
    \end{subfigure}
    \caption{Distribution of $\phi^{*}_{\eta}$ at reconstructed and truth level, for ggF (left) and VBF (right) production modes. The distributions are normalised to 1.}
    \label{phistar}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_ggf_CutTrigger_phistar_resolution.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_vbf_CutTrigger_phistar_resolution.eps}
    \end{subfigure}
 %   \begin{subfigure}[b]{0.49\textwidth}
 %       \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_vbf_CutTrigger_phistar_resolution.eps}
 %   \end{subfigure}
 %   \begin{subfigure}[b]{0.49\textwidth}
 %       \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_vbf_CutTrigger_phistarCS_resolution.eps}
 %   \end{subfigure}
    \caption{Experimental resolution of $\phi^{*}_{\eta}$, for ggF (left) and VBF (right) production modes. The distributions are normalised to 1.}
    \label{resol_phistar}
\end{figure}

We now want to compare the resolutions of $\phi^{*}$ and some other dileptonic variables. We made the choice to concentrate on the vector sum of the leptons' momenta p$_{T}^{ll}$. The resolution of this variable is then expected to be quite poor compared to $\phi^{*}_{\eta}$.\\
Figure \ref{resol} shows this comparison of resolutions as a function of each variable, for VBF and ggF production modes. It shows indeed that the resolution is much worse for p$_{T}^{ll}$ on the whole range, the mean |$\delta$| being roughly one order of magnitude bigger than for $\phi^{*}_{\eta}$.\\
%Additionally, the curves for $\phi^{*}_{\eta}$ and $\phi^{*}_{CS}$ are much closer than what we could expect from Figure \ref{resol_phistar}. The |$\delta$| values are compatible for most of the range, $\phi^{*}_{\eta}$ getting only better for low values (e.g. $\phi^{*}_{\eta}\times(\sqrt{2}M_{Z})\leq$ 50 GeV).

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_ggfresolution.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/H125_tautaull_vbfresolution.eps}
    \end{subfigure}
    \caption{Mean resolution of the two candidate variables as a function of the variable (at reconstructed level), for ggF (left) and VBF (right) production modes.}
    \label{resol}
\end{figure}


\subsubsection{$\phi^{*}$ discrimination power} \label{sec_discri}

H$\rightarrow\tau\tau$ is the best channel to study higgs boson couplings to fermions. Indeed, despite a lower branching ratio than H$\rightarrow$bb, it has a clearer experimental signature, enabling thus to exploit the main two production modes: ggF and VBF.\\
The H$\rightarrow\tau_{lep}\tau_{lep}$ process is of course subject to backgrounds. These can have different causes. Either a pair of leptonically decaying tau leptons is actually produced in the event, or  a process will produce prompt leptons which cannot be, as such, differentiated from leptons coming from tau decay. The main background processes are:
\begin{itemize}
\item Z$\rightarrow\tau\tau$, irreducible background, ranking among the biggest background contributions. It can be discriminated thanks to the invariant mass of the boson (m$_{Z}$ vs m$_{H}$);
\item Z$\rightarrow\ell\ell$, production of two prompt leptons (e or $\mu$). Can also be discriminated with the invariant mass of the boson, as well as with the structure of the events (no tau decay so no or little missing transverse energy for instance);
\item top backgrounds, including $t\bar{t}$ and single top production. In such event there can either be true tau leptons (t$\rightarrow W(\rightarrow \tau\nu)b$) or prompt leptons, or even narrow jets faking leptons. It can be highly limited by requiring events to have no b-jets (\textit{b-veto});
\item Fakes, where jets are recorded as leptons. In this are included several processes, such as W+jet and QCD events.
\end{itemize}

The goal is here to compare the $\phi^{*}_{\eta}$ distribution for the two H$\rightarrow\tau_{lep}\tau_{lep}$ production modes considered, and for the backgrounds described above. The fakes being data-driven, they cannot be shown here and will therefore not be considered.\\
We want as a first step to carry out this comparison for a loose selection, in order to evaluate the overall potential discrimination power. This loose selection will be referred to as the pre-selection in the following. It is defined as follow:
\begin{itemize}
\item At least one primary vertex is required;
\item Hadronically decaying tau leptons are vetoed;
\item We select events with exactly two leptons, having activated the chosen triggers and satisfying the corresponding transverse momenta conditions (typically bigger than 20 GeV).
\end{itemize}
The corresponding plots are shown in Figure \ref{discri_presel}. The first takeaway from these is that the VBF and ggF signal behave clearly differently. Indeed, the distribution for ggF is much more peaked around zero, which would indicate that back-to-back leptons are more likely in this production mode.\\
This is actually to be expected. The Higgs boson transverse momentum is indeed more likely to take high values in the VBF production mode. The tau leptons from the Higgs decay are therefore more likely to be produced collimated than in the ggF case. Since $\phi^{*}_{\eta}$ estimates the "back-to-backness" of the two leptons it is as a consequence less likely to take values around zero.\\
\\
We can then compare each signal with the different backgrounds. Two main features appear, which could be useful to select signals with higher purity:
\begin{itemize}
\item The distribution for ggF is much more peaked around zero than the distributions for top processes (t$\bar{t}$ and single-top) and for the electroweak production modes of Z$\rightarrow\tau\tau$ and Z$\rightarrow\ell\ell$. So by selecting the low-|$\phi^{*}_{\eta}$| region, it would be possible to suppress these backgrounds much more than the ggF signal. We should however note that the distribution for QCD production of Z+jets is even more peaks than the signal, so such a selection would enhance these backgrounds more than the signal. Since they are expected to be the most prominent backgrounds of the analysis, the proposed cut wouldn't have a clear positive impact, potentially even negative.
\item This peaked distribution for Z+jets backgrounds could however be used in the case of VBF signal. Indeed, as stated before, the distribution for VBF is broader, so by cutting away the low-|$\phi^{*}_{\eta}$| we would suppress much more background than signal, and therefore increase the purity.
\end{itemize}

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/ZllS22_CutTrigger_phistar_reco.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/ZllEW_CutTrigger_phistar_reco.eps}
    \end{subfigure}
        \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/ZttS22_CutTrigger_phistar_reco.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/ZttEW_CutTrigger_phistar_reco.eps}
    \end{subfigure}
        \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/ttb_CutTrigger_phistar_reco.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/stop_CutTrigger_phistar_reco.eps}
    \end{subfigure}
    \caption{H$\rightarrow\tau_{lep}\tau_{lep}$ $\phi^{*}_{\eta}$ distribution for ggF and VBF production modes compared to several backgrounds, at pre-selection.}
    \label{discri_presel}
\end{figure}

We have now determined selections which could help increasing the purity of H$\rightarrow\tau_{lep}\tau_{lep}$ signals. This has however been made with a very loose selection, so the question is now to know if these improvements would still be possible in the actual search for H$\rightarrow\tau\tau$ analysis. We will for this consider the same plots, but this time in the signal regions of the analysis, which are much more restrictive. The signal is actually split into two categories, VBF and Boosted, respectively aiming at selecting events from VBF and ggF production modes.\\
The results for the VBF category are given in Figure \ref{discri_VBF}. We focus here on Z+jets backgrounds, since it's for them that we have identified possible improvement for VBF signal. The conclusion from pre-selection is however no more valid in this case. Indeed, the signal region selection have already cut away events with |$\phi^{*}_{\eta}$| around zero. The remaining Z$\rightarrow\tau\tau$ and Z$\rightarrow\ell\ell$ events have nearly the same behaviour as the signal, so we cannot perform better discrimination using $\phi^{*}_{\eta}$ in this signal category.\\
The same way, we look in the Boosted category to the backgrounds for which we had identified potential improvement for ggF signal, i.e. top and electroweak Z+jets. In this case also, the conclusions from pre-selection are not as promising as they were. However, there are still shape differences remaining, especially for $t\bar{t}$ and single backgrounds. $\phi^{*}_{\eta}$ might there bring some additional separation power if used as an input variable of a BDT aiming at selecting events in the Boosted category. 

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/ZllS22_CutVBFCat_phistar_reco.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/ZttS22_CutVBFCat_phistar_reco.eps}
    \end{subfigure}
    \caption{H$\rightarrow\tau_{lep}\tau_{lep}$ $\phi^{*}_{\eta}$ distribution for ggF and VBF production modes compared to several backgrounds, in the VBF category.}
    \label{discri_VBF}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/ZllEW_CutBoostedCat_phistar_reco.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/ZttEW_CutBoostedCat_phistar_reco.eps}
    \end{subfigure}
        \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/ttb_CutBoostedCat_phistar_reco.eps}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{phistar/figures/Taus/stop_CutBoostedCat_phistar_reco.eps}
    \end{subfigure}
    \caption{H$\rightarrow\tau_{lep}\tau_{lep}$ $\phi^{*}_{\eta}$ distribution for ggF and VBF production modes compared to several backgrounds, in the boosted category.}
    \label{discri_boost}
\end{figure}

